Lifting Vectorial Variational Problems: A Natural Formulation based on Geometric Measure Theory and Discrete Exterior Calculus

Numerous tasks in imaging and vision can be formulated as variational problems over vector-valued maps. We approach the relaxation and convexification of such vectorial variational problems via a lifting to the space of currents. To that end, we recall that functionals with polyconvex Lagrangians can be reparametrized as convex one-homogeneous functionals on the graph of the function. This leads to an equivalent shape optimization problem over oriented surfaces in the product space of domain and codomain. A convex formulation is then obtained by relaxing the search space from oriented surfaces to more general currents. We propose a discretization of the resulting infinite-dimensional optimization problem using Whitney forms, which also generalizes recent "sublabel-accurate" multilabeling approaches.

==> figures/illu.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=2.5*1.15in,
height=1.6*1.15in,
at={(0.772in,0.953in)},
scale only axis,
xmin=0,
xmax=1,
xtick={0,0.04,0.08,0.12,0.16,0.2,0.24,0.28,0.32,0.36,0.4,0.44,0.48,0.52,0.56,0.6,0.64,0.68,0.72,0.76,0.8,0.84,0.88,0.92,0.96,1},
xticklabels={\empty},
ymin=0.28,
ymax=0.92,
ytick={0,0.04,0.08,0.12,0.16,0.2,0.24,0.28,0.32,0.36,0.4,0.44,0.48,0.52,0.56,0.6,0.64,0.68,0.72,0.76,0.8,0.84,0.88,0.92,0.96,1},
yticklabels={\empty},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
axis x line=bottom,
axis y line=left,
legend style={legend cell align=left, align=left, draw=white!15!black},
xlabel={$\cX$},
ylabel={$\cY$},
xlabel near ticks,
ylabel near ticks,
scale=1
]

\addplot [color=orange, line width=3pt, opacity=0.33]
  table[row sep=crcr]{%
0	0.804\\
0.00028648979875745	0.799767464841852\\
0.00121395742816743	0.792953871073983\\
0.0027871044430321	0.784853446000559\\
0.00497604074689795	0.775948754822535\\
0.00791347067795511	0.765977645975945\\
0.0114052476543786	0.755747139337352\\
0.0155293367992461	0.745062800374305\\
0.0202262816796527	0.734131507773012\\
0.0257481813691687	0.722472051080423\\
0.0317667315135999	0.710847662729427\\
0.0381799993086075	0.699413758966465\\
0.0453494165529378	0.687550601427023\\
0.0533012269315527	0.675308126371828\\
0.0614870772027507	0.663532116160949\\
0.0703969855737622	0.651511570528293\\
0.0800444798147155	0.639290962933059\\
0.089723841202069	0.627744439459932\\
0.100061759311864	0.616100235600855\\
0.111062716133114	0.60439588125064\\
0.122729056645432	0.59266910017236\\
0.135060981261039	0.580957688411641\\
0.147106357051007	0.570129563946749\\
0.159720764782367	0.559377333166968\\
0.172899414181863	0.548730878290402\\
0.186635946855829	0.538219787566518\\
0.200922453961202	0.527873273045535\\
0.215749498185504	0.517720089393331\\
0.231106139974684	0.507788453977498\\
0.246979967935938	0.498105968446632\\
0.262079819994861	0.48941271245763\\
0.277596614443512	0.48097527322014\\
0.293517412368028	0.472813631658843\\
0.309828318123155	0.464947115574592\\
0.326514512238886	0.457394353873735\\
0.343560286514852	0.450173232452505\\
0.360949081219322	0.443300851840951\\
0.37866352430475	0.43679348670672\\
0.396685472546979	0.43066654731458\\
0.414996054510701	0.424934543032961\\
0.433575715239398	0.419611047973936\\
0.452404262563959	0.414708668848003\\
0.471460914920296	0.410239015109797\\
0.490724350562714	0.406212671465434\\
0.510172758056511	0.402639172806581\\
0.529783887930214	0.399526981630632\\
0.549535105365145	0.396883468000438\\
0.569403443797542	0.394714892091063\\
0.589365659306287	0.393026389364902\\
0.609398285657454	0.391821958410253\\
0.62947768987533	0.391104451472152\\
0.649580128208284	0.390875567697898\\
0.669681802356986	0.391135849113255\\
0.689758915831791	0.391884679338868\\
0.70978773030584	0.393120285049927\\
0.729744621830425	0.394839740175624\\
0.749606136779491	0.397038972828459\\
0.769349047390791	0.399712774946988\\
0.788950406772173	0.402854814629167\\
0.808387603242724	0.406457651127104\\
0.827638413880094	0.410512752467688\\
0.846681057147189	0.415010515657382\\
0.865494244473615	0.419940289423332\\
0.884057230669702	0.425290399436925\\
0.902349863053746	0.431048175960079\\
0.920352629176106	0.437199983848791\\
0.938046703027163	0.44373125484288\\
0.955413989619687	0.450626522065474\\
0.972437167840065	0.457869456650533\\
0.989099731466889	0.465442906411675\\
1	0.470666666666667\\
};

\addplot[-Straight Barb, color=black, line width=0.4pt, point meta={sqrt((\thisrow{u})^2+(\thisrow{v})^2)}, point meta min=0, quiver={scale arrows=0.8,u=\thisrow{u}, v=\thisrow{v}, every arrow/.append style={-{Straight Barb[angle'=18.263, scale={(3/1000)*\pgfplotspointmetatransformed}]}}}]
 table[row sep=crcr] {%
x	y	u	v\\
0.0192307692307692	0.860576923076923	0.0179089095037579	-1.11253052281048e-11\\
0.0192307692307692	0.82051282051282	0.0302013606665955	-0.0534002412856241\\
0.0192307692307692	0.780448717948718	0.0207608279699096	-0.0457601548045786\\
0.0192307692307692	0.740384615384615	0.00846837680707197	-0.0379434438497827\\
0.0192307692307692	0.700320512820513	0.0106943146037645	-0.0379434438602041\\
0.0192307692307692	0.66025641025641	0.0166846039375925	-0.0277928289274772\\
0.0192307692307692	0.620192307692308	0.0085518266135979	-0.0154320752329822\\
0.0192307692307692	0.580128205128205	0.00340396421053175	-0.00643640987729221\\
0.0192307692307692	0.540064102564103	0.00105236354935711	-0.00198380285908123\\
0.0192307692307692	0.5	0.000248258193798811	-0.000436687056468719\\
0.0592948717948718	0.860576923076923	0.00561153745028254	-2.00620987518061e-11\\
0.0592948717948718	0.82051282051282	0.0132516239417483	-0.0161186719170869\\
0.0592948717948718	0.780448717948718	0.015456797456683	-0.0247708032319075\\
0.0592948717948718	0.740384615384615	0.00781671096521725	-0.0282988034191457\\
0.0592948717948718	0.700320512820513	0.0101506149431482	-0.0282988034379588\\
0.0592948717948718	0.66025641025641	0.0225113686480642	-0.0323551280272581\\
0.0592948717948718	0.620192307692308	0.0213564190710267	-0.0276269398588618\\
0.0592948717948718	0.580128205128205	0.0134482723947419	-0.0167731934381027\\
0.0592948717948718	0.540064102564103	0.00599972284166293	-0.00713939060551587\\
0.0592948717948718	0.5	0.00191933445713438	-0.00207328237065146\\
0.0592948717948718	0.459935897435897	0.000431028201006484	-0.000386505482041715\\
0.0993589743589744	0.860576923076923	0.00179023762550046	-1.54667522445357e-11\\
0.0993589743589744	0.82051282051282	0.00543055749232635	-0.00503504813892825\\
0.0993589743589744	0.780448717948718	0.00858069650547245	-0.0111159443843991\\
0.0993589743589744	0.740384615384615	0.00494037663864656	-0.0162950340279282\\
0.0993589743589744	0.700320512820513	0.00663799003327822	-0.0162950340425319\\
0.0993589743589744	0.66025641025641	0.0173564675543154	-0.0228282208870483\\
0.0993589743589744	0.620192307692308	0.0241337612403786	-0.0281995093525818\\
0.0993589743589744	0.580128205128205	0.0238915135015024	-0.0255170532946552\\
0.0993589743589744	0.540064102564103	0.0157522746544323	-0.0155481963308261\\
0.0993589743589744	0.5	0.00700114335489579	-0.00615246702054977\\
0.0993589743589744	0.459935897435897	0.00207575080597731	-0.00148904382301504\\
0.0993589743589744	0.419871794871795	0.000389959083743369	-0.000192190116193083\\
0.139423076923077	0.860576923076923	0.000576489341289588	-1.11093934810986e-11\\
0.139423076923077	0.82051282051282	0.00213567960187596	-0.00160362442756969\\
0.139423076923077	0.780448717948718	0.0041968115968773	-0.00461407189672199\\
0.139423076923077	0.740384615384615	0.00263762133629092	-0.0082773352610451\\
0.139423076923077	0.700320512820513	0.00361742811323563	-0.00827733527183135\\
0.139423076923077	0.66025641025641	0.010606893367222	-0.0131480000858015\\
0.139423076923077	0.620192307692308	0.0186675866926273	-0.0200453264903671\\
0.139423076923077	0.580128205128205	0.0260995854457046	-0.0255944115565702\\
0.139423076923077	0.540064102564103	0.0253643091449747	-0.0227725383873716\\
0.139423076923077	0.5	0.0159784869941508	-0.0126973976426516\\
0.139423076923077	0.459935897435897	0.00639130513456746	-0.00411696978849693\\
0.139423076923077	0.419871794871795	0.00154418911673162	-0.000669323612003013\\
0.139423076923077	0.379807692307692	0.000197848207784618	-3.50308460077719e-05\\
0.179487179487179	0.860576923076923	0.000186613219432565	-6.36054114208912e-12\\
0.179487179487179	0.82051282051282	0.000816485627857134	-0.000515871538580099\\
0.179487179487179	0.780448717948718	0.00190698569353258	-0.00183015381592024\\
0.179487179487179	0.740384615384615	0.00127711328510801	-0.00388903422250161\\
0.179487179487179	0.700320512820513	0.00176732523009519	-0.00388903422959661\\
0.179487179487179	0.66025641025641	0.00558847635735427	-0.00669640666803307\\
0.179487179487179	0.620192307692308	0.0116873497911848	-0.0118198580592588\\
0.179487179487179	0.580128205128205	0.0211643016260726	-0.0190902470845424\\
0.179487179487179	0.540064102564103	0.028649288589925	-0.0239296775849062\\
0.179487179487179	0.5	0.0256567119753438	-0.0192364775436398\\
0.179487179487179	0.459935897435897	0.0141038248581984	-0.00864351448022039\\
0.179487179487179	0.419871794871795	0.00447189804780371	-0.00182634294432308\\
0.179487179487179	0.379807692307692	0.000710390931514104	-0.000106032781671028\\
0.219551282051282	0.82051282051282	0.00030552580525506	-0.000166819510353652\\
0.219551282051282	0.780448717948718	0.000823648927033837	-0.000703908856740541\\
0.219551282051282	0.740384615384615	0.000578740936798843	-0.00173104381175416\\
0.219551282051282	0.700320512820513	0.000810055681893219	-0.0017310438146603\\
0.219551282051282	0.66025641025641	0.00267606955174917	-0.0031303644703013\\
0.219551282051282	0.620192307692308	0.006273746290309	-0.00607306376137478\\
0.219551282051282	0.580128205128205	0.0139897659342486	-0.0117973471410243\\
0.219551282051282	0.540064102564103	0.0252180787000685	-0.0194314040552491\\
0.219551282051282	0.5	0.0312646501130273	-0.0222220440504287\\
0.219551282051282	0.459935897435897	0.0238014397480739	-0.0142443851886494\\
0.219551282051282	0.419871794871795	0.0100816708294697	-0.00405337045641614\\
0.219551282051282	0.379807692307692	0.00202419119809189	-0.000262271015719311\\
0.259615384615385	0.82051282051282	0.00011257677236398	-5.40812209387395e-05\\
0.259615384615385	0.780448717948718	0.000342761397602427	-0.000264383566613808\\
0.259615384615385	0.740384615384615	0.000249978332978842	-0.000738820892259199\\
0.259615384615385	0.700320512820513	0.000368004577356737	-0.000738820890895241\\
0.259615384615385	0.66025641025641	0.00124645641644327	-0.00139144326021901\\
0.259615384615385	0.620192307692308	0.00302036712626523	-0.00283983119674229\\
0.259615384615385	0.580128205128205	0.00780596133800352	-0.00624976753053539\\
0.259615384615385	0.540064102564103	0.0182245916863262	-0.0129920588818386\\
0.259615384615385	0.5	0.0308437308477488	-0.020457576894714\\
0.259615384615385	0.459935897435897	0.0322724984580155	-0.0188915915490168\\
0.259615384615385	0.419871794871795	0.0184540122265375	-0.00751008940132077\\
0.259615384615385	0.379807692307692	0.00476376140718393	-0.000543801300690188\\
0.259615384615385	0.33974358974359	0.000299062426414524	-2.42911909840428e-11\\
0.299679487179487	0.780448717948718	0.000138909251965507	-9.75164140825854e-05\\
0.299679487179487	0.740384615384615	0.000104303609716823	-0.000304950786990736\\
0.299679487179487	0.700320512820513	0.000157433311201564	-0.000304950783523919\\
0.299679487179487	0.66025641025641	0.000575059243161205	-0.000630968194404178\\
0.299679487179487	0.620192307692308	0.00141542201724484	-0.0013718472748449\\
0.299679487179487	0.580128205128205	0.00383753824640434	-0.00296974292327896\\
0.299679487179487	0.540064102564103	0.0110102693331437	-0.00728139392176935\\
0.299679487179487	0.5	0.0253651174431029	-0.015488854696048\\
0.299679487179487	0.459935897435897	0.0367489272387206	-0.0207040736831172\\
0.299679487179487	0.419871794871795	0.0284294610750491	-0.011882302447569\\
0.299679487179487	0.379807692307692	0.00953428057237353	-0.00096278173830084\\
0.299679487179487	0.33974358974359	0.000659156469147796	-5.35946470501893e-11\\
0.33974358974359	0.740384615384615	4.2543956374004e-05	-0.000122597187546146\\
0.33974358974359	0.700320512820513	4.19871630057437e-05	-0.000122597181181554\\
0.33974358974359	0.66025641025641	0.000179559918175689	-0.00026931735842577\\
0.33974358974359	0.620192307692308	0.000681592390432634	-0.000656913459663546\\
0.33974358974359	0.580128205128205	0.00189641468411409	-0.00145929784846154\\
0.33974358974359	0.540064102564103	0.00570547990659225	-0.00353656226386639\\
0.33974358974359	0.5	0.0174210510794374	-0.00959937557753311\\
0.33974358974359	0.459935897435897	0.0358790506995309	-0.0189833060147138\\
0.33974358974359	0.419871794871795	0.0381953041643896	-0.0164623249543474\\
0.33974358974359	0.379807692307692	0.0166460637941933	-0.00147823523328223\\
0.33974358974359	0.33974358974359	0.00126184411603759	-8.60819398925264e-11\\
0.379807692307692	0.620192307692308	0.000225441514455352	-0.000212577183173627\\
0.379807692307692	0.580128205128205	0.000957889429435492	-0.000712683433564931\\
0.379807692307692	0.540064102564103	0.00287019159130012	-0.0017858261262866\\
0.379807692307692	0.5	0.00991837367948398	-0.00481726044854874\\
0.379807692307692	0.459935897435897	0.0298859778491355	-0.01414513538323\\
0.379807692307692	0.419871794871795	0.0459345318437096	-0.0204142186186075\\
0.379807692307692	0.379807692307692	0.0259966054278672	-0.0019982138383655\\
0.379807692307692	0.33974358974359	0.00213739165129988	-9.59304620725673e-11\\
0.419871794871795	0.580128205128205	0.000323165743745857	-0.000233503001366143\\
0.419871794871795	0.540064102564103	0.00160090289434148	-0.000932868915831229\\
0.419871794871795	0.5	0.00506174182522324	-0.00252203622802294\\
0.419871794871795	0.459935897435897	0.020282092532202	-0.00737639996323929\\
0.419871794871795	0.419871794871795	0.0503422257119841	-0.0229659212913577\\
0.419871794871795	0.379807692307692	0.0370602823195999	-0.00240694655594478\\
0.419871794871795	0.33974358974359	0.00326005788861075	-5.68002276566698e-11\\
0.459935897435897	0.540064102564103	0.000581658436227377	-0.000319004959625442\\
0.459935897435897	0.5	0.00347484270365082	-0.00151955348669997\\
0.459935897435897	0.459935897435897	0.00944209285737407	-0.00389800186118128\\
0.459935897435897	0.419871794871795	0.0509039853225777	-0.0119022443729421\\
0.459935897435897	0.379807692307692	0.048962526733998	-0.0118747416962455\\
0.459935897435897	0.33974358974359	0.00454433814071201	-4.34429305953851e-11\\
0.5	0.540064102564103	0.000131284576400234	-6.61355954504253e-05\\
0.5	0.5	0.00148274513078609	-0.000571921868203731\\
0.5	0.459935897435897	0.00989940185307316	-0.003168257916859\\
0.5	0.419871794871795	0.0423654860840328	-0.00409309402008494\\
0.5	0.379807692307692	0.0489625268562119	-0.0151608603398958\\
0.5	0.33974358974359	0.0151347996077966	-3.85812552087798e-11\\
0.540064102564103	0.5	0.000372720808526413	-0.000119284042974579\\
0.540064102564103	0.459935897435897	0.00592092113176723	-0.00146564068712483\\
0.540064102564103	0.419871794871795	0.0389113833258133	-0.00788686182066002\\
0.540064102564103	0.379807692307692	0.0530556211417739	-0.00713104707150394\\
0.540064102564103	0.33974358974359	0.0197051986551626	-1.59448302357026e-11\\
0.580128205128205	0.459935897435897	0.00213182497428259	-0.000349344802786537\\
0.580128205128205	0.419871794871795	0.036700080598544	-0.00591030632626825\\
0.580128205128205	0.379807692307692	0.0568493895598169	-0.00405212415444303\\
0.580128205128205	0.33974358974359	0.0222658472159628	-5.18812932611557e-09\\
0.620192307692308	0.419871794871795	0.0352086053427153	-0.00211653896608395\\
0.620192307692308	0.379807692307692	0.0589659236484701	-0.00149147600416735\\
0.620192307692308	0.33974358974359	0.0237573235099197	-5.1835616905926e-09\\
0.66025641025641	0.419871794871795	0.0352086062235007	-4.40390563038003e-10\\
0.66025641025641	0.379807692307692	0.0589659249714746	0.00229639366551567\\
0.66025641025641	0.33974358974359	0.0237573241435539	4.75398793985458e-12\\
0.700320512820513	0.419871794871795	0.0375050009559639	3.50169993646553e-11\\
0.700320512820513	0.379807692307692	0.0589659260413456	0.0075509964116522\\
0.700320512820513	0.33974358974359	0.021460931509777	2.63115031118597e-12\\
0.740384615384615	0.419871794871795	0.0427596049732423	1.81884679146439e-10\\
0.740384615384615	0.379807692307692	0.0589659272771623	0.0134919949444463\\
0.740384615384615	0.33974358974359	0.0162063305257417	-6.28326402473086e-12\\
0.780448717948718	0.419871794871795	0.0509969985631951	0.00328348092739699\\
0.780448717948718	0.379807692307692	0.05896592851594	0.0162063109697024\\
0.780448717948718	0.33974358974359	0.00796894092961931	-1.77803891836733e-11\\
0.82051282051282	0.459935897435897	0.00332927500508369	1.54609760184146e-05\\
0.82051282051282	0.419871794871795	0.0589605406552156	0.0181378715062191\\
0.82051282051282	0.379807692307692	0.0556824490201293	0.00796891876858149\\
0.860576923076923	0.459935897435897	0.0181836681041244	2.6552309095602e-05\\
0.860576923076923	0.419871794871795	0.0589504586076483	0.0333851107614965\\
0.860576923076923	0.379807692307692	0.0408280629000229	-6.65481550039779e-12\\
0.900641025641026	0.459935897435897	0.0367143890471043	4.31217128408511e-05\\
0.900641025641026	0.419871794871795	0.0589339896990279	0.0408280299070838\\
0.900641025641026	0.379807692307692	0.0222973497847799	1.62538253557319e-08\\
0.940705128205128	0.459935897435897	0.0590116996441323	0.0270098480582362\\
0.940705128205128	0.419871794871795	0.058907353855604	0.0222973098737385\\
0.980769230769231	0.5	0.0270875738224056	-3.26558502726529e-10\\
0.980769230769231	0.459935897435897	0.0590117002160233	0.0589074008754272\\
0.980769230769231	0.419871794871795	0.0319241743129937	7.85033488973095e-08\\
};


\addplot [color=black, dashed, line width=1.5pt, opacity=0.33]
  table[row sep=crcr]{%
0.0192307692307693	0.735446539452103\\
0.0592948717948718	0.671689751587036\\
0.0993589743589743	0.620392202733443\\
0.139423076923077	0.578664145357455\\
0.17948717948718	0.544151028430836\\
0.219551282051282	0.515173727591239\\
0.259615384615385	0.490625088686463\\
0.299679487179487	0.469703420067206\\
0.33974358974359	0.451821694200728\\
0.379807692307692	0.436709644055011\\
0.419871794871795	0.424117081327784\\
0.459935897435897	0.41383878616644\\
0.5	0.405589383217778\\
0.540064102564103	0.399383717481577\\
0.580128205128205	0.395175208543582\\
0.620192307692308	0.392906476318116\\
0.66025641025641	0.392897315846282\\
0.700320512820513	0.394327193995136\\
0.740384615384615	0.397609880859953\\
0.780448717948718	0.402763564205769\\
0.82051282051282	0.409807374365846\\
0.860576923076923	0.419107895152218\\
0.900641025641026	0.43071269144993\\
0.940705128205128	0.444680590682882\\
0.980769230769231	0.461563724718873\\
};

\end{axis}

\end{tikzpicture}%
